BUDHIES I: characterizing the environments in and around two clusters at z~0.2

We present the optical spectroscopy for the Blind Ultra Deep HI Environmental Survey (BUDHIES). With the Westerbork Synthesis Radio Telescope, BUDHIES has detected HI in over 150 galaxies in and around two Abell clusters at z~0.2. With the aim of characterizing the environments of the HI-detected galaxies, we obtained multi-fiber spectroscopy with the William Herschel Telescope. In this paper, we describe the spectroscopic observations, report redshifts and EW[OII] measurements for ~600 galaxies, and perform an environmental analysis. In particular, we present cluster velocity dispersion measurements for 5 clusters and groups in the BUDHIES volume, as well as a detailed substructure analysis.

==> movs/views_2192.tex <==
VIEW={Clearly separated sub-structures}
  C2C=0.6775134205818176 -0.011514212936162949 0.735420286655426
  ROO=5.259204319286711
  ROLL=-54.62416126451559
  BGCOLOR=1. 1. 1.
  LIGHTS=CAD
  RENDERMODE=Solid
END

VIEW={RA-DEC}
  C2C=-0.004025298170745373 0.0665338933467865 -0.9977760314941406
  ROO=5.259204276576638
  ROLL=149.83940593617578
  BGCOLOR=1. 1. 1.
  LIGHTS=CAD
  RENDERMODE=Solid
END

VIEW={DEC-redshift}
  C2C=0.999765157699585 0.005883622448891401 0.020855534821748734
  ROO=5.78512421364566
  ROLL=0.7963772187784496
  BGCOLOR=1. 1. 1.
  LIGHTS=CAD
  RENDERMODE=Solid
END


==> movs/views_963.tex <==
VIEW={Facing A963 1}
  C2C=-0.01015183050185442 0.03894338384270668 -0.9991898536682129
  ROO=6.363637395290967
  ROLL=133.9468534734984
  BGCOLOR=1. 1. 1.
  LIGHTS=CAD
  RENDERMODE=Solid
END

VIEW={Facing A963 2}
  C2C=0.00728618772700429 -0.0030467635951936245 0.9999688267707825
  ROO=6.363637540367901
  ROLL=-74.98498591617486
  BGCOLOR=1. 1. 1.
  LIGHTS=CAD
  RENDERMODE=Solid
END

VIEW={A963_1 and A963_2 along z}
  C2C=-0.04385646432638168 0.9989466667175293 0.013496551662683487
  ROO=5.259210843099081
  ROLL=-85.80908039202838
  BGCOLOR=1. 1. 1.
  LIGHTS=CAD
  RENDERMODE=Solid
END

